Predicting Long Term Sequential Policy Value Using Softer Surrogates

Off-policy policy evaluation (OPE) estimates the outcome of a new policy using historical data collected from a different policy. However, existing OPE methods cannot handle cases when the new policy introduces novel actions. This issue commonly occurs in real-world domains, like healthcare, as new drugs and treatments are continuously developed. Novel actions necessitate on-policy data collection, which can be burdensome and expensive if the outcome of interest takes a substantial amount of time to observe--for example, in multi-year clinical trials. This raises a key question of how to predict the long-term outcome of a policy after only observing its short-term effects? Though in general this problem is intractable, under some surrogacy conditions, the short-term on-policy data can be combined with the long-term historical data to make accurate predictions about the new policy's long-term value. In two simulated healthcare examples--HIV and sepsis management--we show that our estimators can provide accurate predictions about the policy value only after observing 10\% of the full horizon data. We also provide finite sample analysis of our doubly robust estimators.

==> arxiv_dec_2024/experiment_results.tex <==

\begin{table}[h]
\centering
\caption{We show the estimation error on the HIV simulator at different short horizons. (Pick which h's to include in the main text.)}
\begin{tabular}{@{}lcc@{}}
\toprule
Estimator & Short horizon (\% of H) & Error 
\\ \midrule
Weighted SLEV   & 2 (1\%) & 66.61    \\
Unweighted SLEV  & 2 (1\%)& 68.3 \\
DR-weighted SLEV & 2 (1\%) & 66.81 \\ 
DR-unweighted SLEV  & 2 (1\%)& 67.16 \\
Dynamics model-based & 2 (1\%)& 404.82 \\ 
Mean reward $\times 200$ & 2 (1\%)& 404.84 \\
Last reward $\times 200$ & 2 (1\%)& 404.81 \\
Historical mean & 0  & 67.86 \\
\midrule 
Weighted SLEV   & 5 (2.5\%) & 61.84   \\
Unweighted SLEV  & 5 (2.5\%)& 68.16 \\
DR-weighted SLEV & 5 (2.5\%) & 57.8 \\ 
DR-unweighted SLEV  & 5 (2.5\%)& 68.16 \\
Dynamics model-based & 5 (2.5\%)& 404.77 \\ 
Mean reward $\times 200$ & 5 (2.5\%)& 404.79 \\
Last reward $\times 200$ & 5 (2.5\%)& 404.71 \\
\midrule 
Weighted SLEV   & 10 (5\%) & 71.51    \\
Unweighted SLEV  & 10 (5\%) & 68.15 \\
DR-weighted SLEV & 10 (5\%) & 70.91 \\ 
DR-unweighted SLEV  & 10 (5\%) & 68.15 \\
Dynamics model-based & 10 (5\%) & 404.58 \\ 
Mean reward $\times 200$ & 10 (5\%) & 404.68 \\
Last reward $\times 200$ & 10 (5\%) & 404.37 \\
\midrule 
Weighted SLEV   & 20 (10\%) & 53.21    \\
Unweighted SLEV  & 20 (10\%) & 67.15 \\
DR-weighted SLEV & 20 (10\%) & 50.61 \\ 
DR-unweighted SLEV  & 20 (10\%) & 64.86 \\
Dynamics model-based & 20 (10\%) & 402.49\\ 
Mean reward $\times 200$ & 20 (10\%) & 403.83 \\
Last reward $\times 200$ & 20 (10\%) & 400.56 \\
\midrule 
Weighted SLEV   & 50 (25\%) & 53.85    \\
Unweighted SLEV  & 50 (25\%) & 57.96 \\
DR-weighted SLEV & 50 (25\%) & 55.26 \\ 
DR-unweighted SLEV  & 50 (25\%) & 58.15 \\
Dynamics model-based & 50 (25\%) & 137.32 \\ 
Mean reward $\times 200$ & 50 (25\%) & 334.36 \\
Last reward $\times 200$ & 50 (25\%) & 31.79 \\ \bottomrule
\end{tabular}
\label{table:hiv_mse}
\end{table}



\begin{table}[h]
\centering
\caption{We show the paired T-statistics using the SLEV estimates to compare the mean values of the behavioral and the new target policies. (*) for significant p values below 0.01.}
\begin{tabular}{@{}lccc@{}}
% \toprule
% Estimator & Short horizon & T-stats (p-value)
% \\ \midrule
% Weighted SLEV   & 20 (10\%) & 30.13*   \\
% Unweighted SLEV  & 20 (10\%)& 1.45 (0.14) \\
% DR-weighted SLEV & 20 (10\%) & 42.54* \\ 
% DR-unweighted SLEV  & 20 (10\%)& 5.95*\\
% \midrule
% Weighted SLEV   & 50 (25\%) & 28.81*   \\
% Unweighted SLEV  & 50 (25\%)& 17.12*\\
% DR-weighted SLEV & 50 (25\%) & 19.55*\\ 
% DR-unweighted SLEV  & 50 (25\%)& 18.03*\\ \bottomrule
\toprule
Estimator & Short horizon & T-stats & p-value (*)
\\ \midrule
Weighted SLEV   & 20 (10\%) & 30.13 & 2.09e-114 (*)   \\
Unweighted SLEV  & 20 (10\%)& 1.45 & 0.14 \\
DR-weighted SLEV & 20 (10\%) & 42.54 & 4.10e-168 (*) \\ 
DR-unweighted SLEV  & 20 (10\%)& 5.95 & 4.98e-9 (*)\\
\midrule
Weighted SLEV   & 50 (25\%) & 28.81 & 3.13e-108 (*)   \\
Unweighted SLEV  & 50 (25\%)& 17.12 & 4.58e-52 (*)\\
DR-weighted SLEV & 50 (25\%) & 19.55 & 1.20e-63 (*)\\ 
DR-unweighted SLEV  & 50 (25\%)& 18.03 & 2.43e-56 (*)\\ \bottomrule
\end{tabular}
\label{table:hiv_tstats}
\end{table}


\begin{table}[h]
\caption{We show the estimation error on the Sepsis simulator at different short horizons. Neutral, pessimistic, optimistic projections use the true returns for patients who entered terminal states by $h$ and project with \{0, 1, -1\} for the remaining patients whose final outcomes are still unknown at $h$.}
\centering
\begin{tabular}{@{}lcc@{}}
\toprule
Estimator  & Short horizon (\% of H) & Error \\ \midrule
Weighted SLEV   & 2 (10\%) & 0.008     \\
Unweighted SLEV  & 2 (10\%) & 0.017   \\
DR-weighted SLEV & 2 (10\%) & 0.049  \\ 
DR-unweighted SLEV & 2 (10\%) & 0.078 \\ 
Dynamics model-based & 2 (10\%) & 0.527 \\
Neutral projection & 2 (10\%) & 0.076 \\ 
Pessimistic projection & 2 (10\%) & 0.759 \\ 
Optimistic projection & 2 (10\%) & 0.912 \\ 
Mean projection & 2 (10\%) & 0.089 \\
\midrule 
Weighted SLEV   & 4 (20\%) & 0.037 \\
Unweighted SLEV   & 4 (20\%)  & 0.020   \\
DR-weighted SLEV & 4 (20\%) & 0.003   \\ 
DR-unweighted SLEV & 4 (20\%) & 0.035 \\ 
Dynamics model-based & 4 (20\%) &  0.369 \\
Neutral projection & 4 (20\%) &  0.077 \\ 
Pessimistic projection & 4 (20\%) & 0.692 \\ 
Optimistic projection & 4 (20\%) & 0.846 \\ 
Mean projection & 4 (20\%) & 0.074 \\
\midrule 
Weighted SLEV   & 5 (25\%) & 0.030 \\
Unweighted SLEV   & 5 (25\%)  & 0.010   \\
DR-weighted SLEV & 5 (25\%) & 0.020   \\ 
DR-unweighted SLEV & 5 (25\%) & 0.0001 \\ 
Dynamics model-based & 5 (25\%) & 0.320 \\
Neutral projection & 5 (25\%) & 0.072 \\ 
Pessimistic projection & 5 (25\%) & 0.680 \\ 
Optimistic projection & 5 (25\%) & 0.824 \\ 
Mean projection &5 (25\%) & 0.074  \\
\bottomrule
\end{tabular}
\label{table:sepsis_error}
\end{table}


\begin{table}[h]
\centering
\caption{We show the independent T-statistics using the SLEV estimates to compare the mean values of the historical and the new policies. (*) for significant p values below 0.01.}
\begin{tabular}{@{}lccc@{}}
% \toprule
% Estimator & Short horizon & T-stats 
% \\ \midrule
% Weighted SLEV   & 2 (10\%) & 16.40*  \\
% Unweighted SLEV  & 2 (10\%)& 19.19* \\
% DR-weighted SLEV & 2 (10\%) & 12.49* \\ 
% DR-unweighted SLEV  & 2 (10\%)& 9.30* \\
% \midrule
% Weighted SLEV   & 4 (20\%) & 12.73* \\
% Unweighted SLEV  & 4 (20\%)& 14.69* \\
% DR-weighted SLEV & 4 (20\%) & 16.96* \\ 
% DR-unweighted SLEV  & 4 (20\%)& 13.17* \\ \bottomrule
\toprule
Estimator & Short horizon & T-stats & p-value (*)
\\ \midrule
Weighted SLEV   & 2 (10\%) & 16.40 & 1.10e-59 (*)   \\
Unweighted SLEV  & 2 (10\%)& 19.19 & 1.07e-80 (*) \\
DR-weighted SLEV & 2 (10\%) & 12.49 & 1.45e-35 (*) \\ 
DR-unweighted SLEV  & 2 (10\%)& 9.30 & 1.68e-20 (*)\\
\midrule
Weighted SLEV   & 4 (20\%) & 12.73 & 7.28e-37 (*)   \\
Unweighted SLEV  & 4 (20\%)& 14.69 & 2.09e-48 (*)\\
DR-weighted SLEV & 4 (20\%) & 16.96 & 1.16e-63 (*)\\ 
DR-unweighted SLEV  & 4 (20\%)& 13.17 & 2.53e-39 (*)\\ \bottomrule
\end{tabular}
\label{table:sepsis_tstats}
\end{table}


==> arxiv_dec_2024/supplement_synthetic.tex <==
We design a low signal-to-ratio environment with surrogates to evaluate the robustness of Short Long Regression estimators to model mis-specification of a density ratio estimator and a regressor. Similarly as before, our goal is to estimate the long-term returns under a new target policy $\pi_2$ only using short-term state trajectories observed under $\pi_2$ and a historical dataset of short-term state trajectories and their corresponding long-term returns under $\pi_b$. First we introduce the synthetic domain details: states, transitions, returns, and surrogacy.

\paragraph{Domain}Initial states $s_0$ are evenly spaced between [0, 1.5] with additive $N(0, 0.1)$ noise. Under $\pi_b$, transitions to the next state are as follows:

\[
s_1 =
\begin{cases} 
s_0 & \text{w.p 0.5} \\
(-0.6 + 0.1 * U[0,1)) * s_0 & \text{w.p 0.45} \\
1.5 & \text{otherwise}
\end{cases}
\] with additive noise from $N(0, 0.1)$.
Under $\pi_2$, the next state is determined deterministically as:
\[
s_1 =
\begin{cases} 
1.5 & \text{if $s_0 < 1.25$} \\
0 & \text{otherwise}
\end{cases}
\]
plus additive noise from $N(0, 0.1)$. The true long-term return $V^{\pi_b} = V^{\pi_2} = f(s_0, s_1)$ with a quadratic function $f(s_0, s_1) = 5 s_0 + s_1 + s_1^2$. The observed return under $\pi_b$ $V^{\pi_b}_{MC} = V^{\pi_b} + N(0, \omega)$ where $\omega$ determines the amount of noise in the delayed returns (i.e., the higher the $\omega$, the more reliable the regression estimates are compared to the Monte Carlo estimates, same amount of noise is applied to the returns under $\pi_2$). $|D_b| = 5000$, and $|D_2| = 100$. 

We fit an ordinary least squares regression model using `statsmodel` packages. A correct regressor given $(s_0, s_1)$ is fitted as: $f_\theta(s_0, s_1) = \theta^\top [s_0, s_1, s_1^2]$. The continuous states are discretized into 50 bins (thus making a total of 2500 bins for $(s_0, s_1)$), and the number of occurrences per bin is counted to estimate the density ratio between $p(s_0, s_1|\pi_2, \mathcal M_2)$ and $p(s_0, s_1|\pi_b, \mathcal M_b)$. We report the mean squared error of the true and the estimated rewards of the 100 target trajectories under $\pi_2$: $\sqrt{\frac{1}{|D_{2}|}\sum_{i=1}^{100} (\hat V^{\pi_2}_i - V^{\pi_2}_i)^2}$. The code for Table 1 is available as ``surrogate synthetic.py" and the remaining experiments with ``surrogate.py" using --Ntrain 5000 --Ntarget 100. 

\begin{table}[h]
\centering
\caption{\textbf{We show the mean and standard deviation of Mean-Squared Error (MSE) with 200 datasets where the randomness comes from the stochastic transitions under $\pi_b$ and gaussian noises.}}
% \begin{tabular}{@{}lcc@{}}
% \toprule
%  & \begin{tabular}[c]{@{}l@{}}Large noise \\ ($\omega = 10$)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Small noise \\ ($\omega = 1$)\end{tabular} \\ \midrule
% Short long estimator with unweighted regressor   & \textbf{0.11 (0.15)}    &   \textbf{0.002 (0.002)}  \\
% Monte Carlo full returns estimate   &  103.63 (11.24)   &  0.99 (0.16)   \\ \bottomrule
% \end{tabular}
\begin{tabular}{@{}lcc@{}}
\toprule
 & \begin{tabular}[c]{@{}l@{}}Large noise \\ ($\omega = 10$)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Small noise \\ ($\omega = 1$)\end{tabular} \\ \midrule
Short long estimator with unweighted regressor   & \textbf{0.251 (0.307)}    &   \textbf{0.002 (0.003)}  \\
Monte Carlo full returns estimate   &  98.457 (13.355)   &  0.984 (0.133)   \\ \bottomrule
\end{tabular}
\label{table:synthetic_noise}
\end{table}

As discussed in the main text, Table \ref{table:synthetic_noise} shows that our estimates using the short trajectory data provides give more accurate predictions of $V^{\pi_2}$ than using a Monte Carlo estimates of the full return $V^{\pi_2}_{MC}$. Here the regressor is correctly specified, and the comparison is only between the surrogate-based regression estimates and the noisy Monte Carlo estimates. 



\paragraph{Model Mis-specification}Next we consider either regressor or density ratio estimator misspecification. A correct regressor is a quadratic function of $s_0, s_1$: $f(s_0, s_1) = 5 s_0 + s_1 + s_1^2$ as stated above, but we use a mis-specified regressor model, in particular a linear model, $f_{\tilde \theta}(s_0, s_1) = {\tilde \theta}^\top [s_0, s_1]$. Note that this linear model can still capture the distribution under $\pi_2$ since $s_1$ under $\pi_2$ is either 0 or 1.5, but not under $\pi_b$. This is by design to show that even when the regression model is mis-specified, when the density ratio estimates are correct, the target estimates can still be accurate as long as the behavioral data supports the target data distribution. We expect the weighted regressor and the doubly robust estimator to be unaffected but the unweighted regressor to fit the target data poorly.

In order to estimate the density ratios, the continuous states are discretized into 50 bins (thus making a total of 2500 bins for $(s_0, s_1)$), and the number of occurrences per bin is counted under $\pi_2$ and under $\pi_b$. Then to  bias the density ratio estimates, we add a non-zero gaussian noise from N(10, 10) to the denominator representing $p(s_0, s_1|\pi_b, \mathcal M_b)$ in the density ratios between $p(s_0, s_1|\pi_2, \mathcal M_2)$  and $p(s_0, s_1|\pi_b, \mathcal M_b)$. We expect the unweighted Short Long Regression estimator and the doubly robust estimator to be unaffected by the density ratio mis-specification as the regressor model is still correct.

\paragraph{Results}
\begin{table}[h]
\centering
\caption{\textbf{We show the MSE of estimators for synthetic example ($\omega = 1$) when regression model or density ratio model may be mis-specified. Mean and std from 200 datasets where the randomness comes from the stochastic transitions under $\pi_b$ and gaussian noises.}}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{@{}lccc@{}}
% \toprule 
%  & Realizable & Regressor Model Misspecified & Density Ratio Model Misspecified \\ \midrule
%  Short long estimator with unweighted regressor  & 0.98 (0.13)   & \textbf{1.89 (0.23)} & 0.98 (0.13) \\
% Short long regression estimator   & 1.07 (0.17)   & 1.07 (0.17)   & \textbf{1.37 (0.71)}  \\ 
% DR short long estimator & 0.99 (0.13)   &  0.99 (0.13) & 0.99 (0.13) \\ \bottomrule
% \end{tabular}}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccc@{}}
\toprule 
 & Realizable & Regressor Model Misspecified & Density Ratio Model Misspecified \\ \midrule
 Short long estimator with unweighted regressor  & 0.002 (0.003)   & \textbf{0.914 (0.064)} & 0.002 (0.003) \\
Short long regression estimator   & 0.079 (0.085)   & 0.080 (0.068)   & \textbf{0.388 (0.728)}  \\ 
DR short long estimator & 0.008 (0.007)   &  0.008 (0.007) & 0.006 (0.005) \\ \bottomrule
\end{tabular}}
% }
\label{table:synthetic_weighted}
\end{table}

Table \ref{table:synthetic_weighted} compares the performance of the 3 different regressors under different conditions. As expected, the doubly robust method does well in all three cases. The short long estimator with weighted regression continues to perform well when the density model is well specified, when fitting a (misspecified) linear regression model, because $V^{\pi_2}$ can be well fit with a linear function. Note however that this method performs less well when the density ratio model is misspecified, since the incorrect weights impact the learned regression model. Note that we consider the use of a linear regression model as misspecification in this case because because the linear model is only correct for the processes under $\pi_2$ and not for the processes under $\pi_b$, which require a quadratic.

Even when the density ratio estimates are incorrect, unweighted and DR estimates perform well when the regressor is correctly specified. Since the regression model itself is still consistent, as the training data size increases, the effect due to the incorrect density ratio estimates is lessened for the weighted short long horizon regression estimate, as we show in  in Table \ref{table:synthetic_weighted2}. 

Our synthetic experiments demonstrate that the doubly robust estimator is robust to both regressor and density ratio estimator misspecification. The unweighted estimator has a higher error when the regression model is misspecified, and the weighted estimator  has higher error when the density ratio model is misspecified (since this impacts the regression fit due to a limited training sample size).

\begin{table}[h]
\centering
\caption{\textbf{MSE using different training data sizes of the short long regression estimator when the density ratio estimates are misspecified.}}
\begin{tabular}{@{}lc@{}}
\toprule
Training data size &  Error \\ \midrule
500  & 2.123 (7.382) \\
1000  & 0.806 (1.281) \\
% 5000 & 1.37 (0.71) \\
% 10000 & 1.27 (0.43) \\
50000 & 0.259 (0.480) \\
 \bottomrule
\end{tabular}
% \begin{tabular}{@{}lc@{}}
% \toprule
% Training data size &  Error \\ \midrule
% 500  & 3.11 (7.27) \\
% 1000  & 1.80 (1.29) \\
% % 5000 & 1.37 (0.71) \\
% % 10000 & 1.27 (0.43) \\
% 50000 & 1.17 (0.42) \\
%  \bottomrule
% \end{tabular}
\label{table:synthetic_weighted2}
\end{table}

% Use $|D_{\text{train}}| = 10000, |D_{\text{train}}| = 100$, and (discretized bins = 50 per dimension) pseudo-counts for density estimates. Initial states $x_0$ are evenly spaced between $[0, 1.5]$. Transition probability of $x_1$ are: With 0.5, probability $x_1 = x_0$, with 0.45 probability, $x_1 = (-.6 + .1 * \text{Unif}(0,1)) * x_0$, and with 0.05 probability set to 1.5 (and iid noise $N(0, \sigma)$ is applied to $x_0, x_1$ separately).

% True surrogates are $X = \{x_0, x_1, x_1^2\}$ (and regressor has 3 degrees of freedom). A correct regressor class is $\theta := \{\theta_0, \theta_1, \theta_2\}$ (which can be estimated via OLS), and the observed returns are $\tilde G = X^\top \theta + N(0, \omega)$. 

% \paragraph{Benefits of utilizing surrogates from historical data over noisy online returns}


% Even when the experimentation budget for full H horizons is available, if the surrogates exist and the offline data size is large (so the large training data can sweep out the mean zero noise), then the short-term surrogate based estimates can give a smaller error than observing the actual on-policy long term returns. We control the noise in the long-term returns via $\tilde G = G + N(0, \omega)$ where $G$ is the true return and $\tilde G$ is the noisy observed return. (Table \ref{table:synthetic_noise}.)

% \paragraph{Benefit of re-weighting surrogates in the case of misspecified regression model}

% Mis-specified surrogates are $\{x_0, x_1\}$ (and the regressor only has 2 degrees of freedom $\{\theta_0, \theta_1\}$), but the second dimensions of the target surrogates are either $0 +  N(0, \sigma)$ or $1.5 + N(0, \sigma)$, so even the best fit using this misspecified model can still be accurate for the test data, but not for the entire train data. 

% If the regression model has 3 degrees of freedom, both weighted and unweighted SLEV give accurate predictions. But if the regression model is mis-specified (for example, only has 2 degrees of freedom), weighted OLS based on density ratio estimates can better fit the test data. (Table \ref{table:synthetic_weighted}.)

% \begin{table}[h]
% \centering
% \begin{tabular}{@{}lcc@{}}
% \toprule
% Domain
% Estimator & Correct   & Misspec \\ \midrule
% Unweighted SLEV   & \textbf{0.93 (0.09)}       &  1.84 (0.16)   \\
% Weighted SLEV     &  1.01 (0.18)      &  \textbf{1.06 (0.12)}  \\ 
% DR SLEV     &      &  \\ \bottomrule
% \end{tabular}
% \caption{We show the Mean-Squared Error (MSE) of a synthetic environment over 10 seeds.}
% \label{table:synthetic_weighted}
% \end{table}


% \paragraph{Benefit of doubly robust estimation in the case of misspecified density model} 

% (Note: because of train set split for density ratio fitting and weight estimation, we set weights to 1 if the train-val point never occurs before, and 0 if it appears only in test-fit, but the second case rarely happens.) 

% Note from the above set up that $\{x, y, x^2, y^2\}$ is also a valid surrogate and the regressor has 4 degrees of freedom although $x^2$ can be completely ignored. We test the robustness of the DR estimator to the incorrect density ratio estimates. A bias is applied to the density ratio estimate as: $\frac{\tilde P_{\text{test}}}{\tilde P_{\text{train}} + N(\beta, 1)}$. Incorrectly weighted SLEV may suffer due to the noise by $x^2$ while unweighted SLEV is unaffected. DR SLEV performs closely to unweighted SLEV estimates despite the bias in the weight estimates. (Table \ref{table:synthetic_dr}.)
% \begin{table}[h]
% \centering
% \begin{tabular}{@{}lccc@{}}
% \toprule
% Domain
% Estimator & $\beta=0.5$ & 1 \\ \midrule
% Weighted SLEV  & 1.25 (0.33) & 1.37 (0.29) \\
% DR SLEV  &  \textbf{0.89 (0.10)} &  1.04 (0.18) \\ 
% Unweighted SLEV  &  \textbf{0.89 (0.10)} & \textbf{1.02 (0.14)} \\ \bottomrule
% \end{tabular}
% % \begin{tabular}{@{}lcccc@{}}
% % \toprule
% % Domain
% % Estimator & No noise   & $\beta=0.5$ & 1 \\ \midrule
% % Weighted SLEV   &  1.07 (0.08)  & 1.25 (0.33) & 1.37 (0.29) \\
% % DR SLEV   & 1.01 (0.09)   &  \textbf{0.89 (0.10)} &  1.04 (0.18) \\ 
% % Unweighted SLEV & 0.99 (0.08) &  \textbf{0.89 (0.10)} & \textbf{1.02 (0.14)} \\ \bottomrule
% % \end{tabular}
% \caption{We show the Mean-Squared Error (MSE) of a synthetic environment over 10 seeds when the propensity weights are biased by $\beta = \{0.5, 1\}$.}
% \label{table:synthetic_dr}
% \end{table}

% \paragraph{Sensitivity to surrogate assumption}

%  In the previous synthetic experiments, we only consider a zero-mean gaussian noise, so the surrogate assumption holds with $h = 2$. When this assumption is violated, similar to the setting by Saito et al., short horizon surrogate-based estimates no longer can give theoretical guarantees, so we empirically explore how sensitive the surrogate-based estimates are to different levels of $\alpha$. (May need to re-generate the plot since the dynamics for the other synthetic examples have changed a bit.)

% \begin{table}[h]
% \centering
% \begin{tabular}{@{}lcc@{}}
% \toprule
% Domain
% Estimator          & Original               & Misspec \\ \midrule
% Unweighted SLEV   & 2.079 (0.03)            & \textbf{2.07 (0.029)}       \\
% Weighted SLEV     & 1.05 (0.31)          & 2.99 (0.9049)                \\
% DR SLEV & \textbf{0.91 (0.20)} & 2.1426 (0.04)                \\ \bottomrule
% \end{tabular}
% \caption{We show the Mean-Squared Error (MSE) of a synthetic environment.}
% \end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figures/synthetic_surrogacy_violation.png}
%     \caption{We show the Mean-Squared Error (MSE) when the surrogacy assumption is violated. $\alpha$=0 means there is no violation, and $\alpha$=1 means the reward is fully policy dependent.}
%     \label{fig:enter-label}
% \end{figure}
